Extreme Consistency: Overcoming Annotation Scarcity and Domain Shifts

Supervised learning has proved effective for medical image analysis. However, it can utilize only the small labeled portion of data; it fails to leverage the large amounts of unlabeled data that is often available in medical image datasets. Supervised models are further handicapped by domain shifts, when the labeled dataset, despite being large enough, fails to cover different protocols or ethnicities. In this paper, we introduce \emph{extreme consistency}, which overcomes the above limitations, by maximally leveraging unlabeled data from the same or a different domain in a teacher-student semi-supervised paradigm. Extreme consistency is the process of sending an extreme transformation of a given image to the student network and then constraining its prediction to be consistent with the teacher network's prediction for the untransformed image. The extreme nature of our consistency loss distinguishes our method from related works that yield suboptimal performance by exercising only mild prediction consistency. Our method is 1) auto-didactic, as it requires no extra expert annotations; 2) versatile, as it handles both domain shift and limited annotation problems; 3) generic, as it is readily applicable to classification, segmentation, and detection tasks; and 4) simple to implement, as it requires no adversarial training. We evaluate our method for the tasks of lesion and retinal vessel segmentation in skin and fundus images. Our experiments demonstrate a significant performance gain over both modern supervised networks and recent semi-supervised models. This performance is attributed to the strong regularization enforced by extreme consistency, which enables the student network to learn how to handle extreme variants of both labeled and unlabeled images. This enhances the network's ability to tackle the inevitable same- and cross-domain data variability during inference.

==> extra.tex <==
% \vspace{4pt}
% \noindent{\bf Our method promotes extreme prediction consistency.} The novelty of our approach lies in the design of the consistency loss. While the existing methods exercise prediction consistency under a limited set of transformations, we take the prediction consistency to extremes through a diverse and advanced set of transformations, which impose numerous invariance and equivariance constraints on the student network. We hypothesize that extreme consistency better utilize the unlabeled data, providing stronger regularization, thereby enabling a higher-performing student network. 

% \vspace{4pt}
% \noindent{\bf Our method reserves exclusive perturbations for the student network.} The key to the success of extreme consistency loss is to secure a quality reference prediction by the teacher network. For this purpose, the teacher network receives as the input either the original unlabeled data without any augmentation or the labeled data with only mild transformations through a basic transformation $T_B$ module. The student network, however, receives as the input a severely transformed image, which is obtained by sending the input of the teacher network through an advanced transformation  $T_A$ module.

% At the core of our methodology The student and teachner To leverage the unlabeled data, we introduce extreme consistency loss, which measures the consistency between the predictions of the student and teacher networks when they receive a severely transformed and a mildly transformed version of a given image, respectively.

% Our method has the following properties:
% Since our method is agnostic to the source of the unlabeled data, it can handle both domain shift problem (where $\mathcal{U}$ comes from a domain other than $\mathcal{L}$) and scarce annotation problem (where $|\mathcal{L}|$ is small and $\mathcal{U}$ and $\mathcal{L}$ belong to the same domain). This capability is attributed to our diverse and exclusive perturbations that bridged both within- and cross-domain data disparity. 

% \vspace{4pt}
% \noindent{\bf Our method can be tailored for various vision tasks.}
% The extreme consistency loss, at the core of our method, can be tailored for  classification, segmentation, and detection by subjecting classification logits, segmentation masks, and saliency maps to the extreme consistency loss, respectively. Note that saliency or center maps are used in recent object detectors such as CenterNet \cite{duan2019centernet}.

% \vspace{4pt}
% \noindent{\bf Our method is a simple and intuitive.} We have presented the pseudocode of our SSL method in Algorithm~\ref{algo:ssl}. Our architecture consists of two networks with an identical architecture: a student network ($N_s$) whose weights are updated through backpropagation during training, and a teacher network ($N_t$) whose weights track the weights of the student network through an exponential moving average filter. The teacher network can be viewed as a temporal ensemble model, which aggregates different snapshots of the student network during the course of training. The student network is trained by minimizing the supervised Dice-based segmentation loss ($L_{seg}$), and an unsupervised consistency loss $L_{cons}$ based on soft Dice, which encourages the student network to generate predictions consistent with the reference predictions by the teacher. 

% \vspace{4pt}
% \noindent{\bf Our method promotes extreme prediction consistency.} The novelty of our approach lies in the design of the consistency loss. While the existing methods exercise prediction consistency under a limited set of transformations, we take the prediction consistency to extremes through a diverse and advanced set of transformations, which impose numerous invariance and equivariance constraints on the student network. We hypothesize that extreme consistency better utilize the unlabeled data, providing stronger regularization, thereby enabling a higher-performing student network. 

% \vspace{4pt}
% \noindent{\bf Our method reserves exclusive perturbations for the student network.} The key to the success of extreme consistency loss is to secure a quality reference prediction by the teacher network. For this purpose, the teacher network receives as the input either the original unlabeled data without any augmentation or the labeled data with only mild transformations through a basic transformation $T_B$ module. The student network, however, receives as the input a severely transformed image, which is obtained by sending the input of the teacher network through an advanced transformation  $T_A$ module. 
